Certifying Euclidean Sections and Finding Planted Sparse Vectors Beyond the $\sqrt{n}$ Dimension Threshold

We consider the task of certifying that a random $d$-dimensional subspace $X$ in $\mathbb{R}^n$ is well-spread - every vector $x \in X$ satisfies $c\sqrt{n} \|x\|_2 \leq \|x\|_1 \leq \sqrt{n}\|x\|_2$. In a seminal work, Barak et. al. showed a polynomial-time certification algorithm when $d \leq O(\sqrt{n})$. On the other hand, when $d \gg \sqrt{n}$, the certification task is information-theoretically possible but there is evidence that it is computationally hard [MW21,Cd22], a phenomenon known as the information-computation gap. In this paper, we give subexponential-time certification algorithms in the $d \gg \sqrt{n}$ regime. Our algorithm runs in time $\exp(\widetilde{O}(n^{\varepsilon}))$ when $d \leq \widetilde{O}(n^{(1+\varepsilon)/2})$, establishing a smooth trade-off between runtime and the dimension. Our techniques naturally extend to the related planted problem, where the task is to recover a sparse vector planted in a random subspace. Our algorithm achieves the same runtime and dimension trade-off for this task.

==> prelims.tex <==
\section{Preliminaries}

\paragraph{Notation.}
For an integer $N$, we will use $[N]$ to denote the set $\{1,2,\dots, N\}$.

% We refer readers to the book by Vershynin~\cite{Ver20} for a thorough exposition.

\begin{definition}[Sub-gaussian variable]
    The sub-gaussian norm of a random variable $X$, denoted $\|X\|_{\psi_2}$, is defined to be
    $\|X\|_{\psi_2} = \inf\{t > 0: \E[\exp(X^2/t^2)] \leq 2\}$.
\end{definition}

There are several equivalent properties of sub-gaussian variables.
\begin{lemma}[Sub-gaussian properties] \label{lem:sub-gaussian}
    Let $X$ be a random variable with sub-gaussian norm $\psi$.
    Then, we have
    \begin{enumerate}[(1)]
        \item $\|X\|_{L^p} = \E[|X|^p]^{1/p} \leq C \psi \sqrt{p}$ for all integers $p \geq 1$;
        \item $\Pr[|X| \geq t] \leq 2 \exp(-t^2/\psi^2)$.
    \end{enumerate}
    Here $C > 0$ is an absolute constant.
\end{lemma}

\begin{fact}[See e.g.~\cite{Ver20}] \label{fact:gaussian-matrix}
    Let $m \leq n$, and let $A \in \R^{n \times m}$ be a matrix with i.i.d.\ $\calN(0,1)$ entries.
    Then, for every $t \geq 0$, with probability at least $1 - 2e^{-t^2/2}$, we have $\sqrt{n} - \sqrt{m} - t \leq \sigma_{\min}(A) \leq \sigma_{\max}(A) \leq \sqrt{n} + \sqrt{m} + t$.
\end{fact}


\subsection{Distortion and Well-spreadness}


\begin{definition}[Distortion of a subspace]
    For a subspace $X \subseteq \R^n$, define the distortion of $X$ to be
    \begin{equation*}
        \Delta(X) = \sup_{x\in X: x\neq 0} \frac{\sqrt{n} \norm{x}_2}{\norm{x}_1} \mper
    \end{equation*}
\end{definition}

It is often more convenient to work with the following notion.

\begin{definition}[Spreadness property of a subspace] \label{def:spread-subspace}
    A subspace $X \subseteq \R^n$ is $(t,\eps)$-spread if for every $x\in X$ and every $S\subseteq [n]$ with $|S| \leq t$, we have
    \begin{equation*}
        \norm*{x_{\ol{S}}}_2 \geq \eps \cdot \norm{x}_2 \mper
    \end{equation*}
\end{definition}

The relationship between the distortion and spread of a subspace was proved in \cite{GuruswamiLR10}.
In particular, it implies that $\Delta(X) = O(1)$ if and only if $X$ is $(\Omega(n),\Omega(1))$-spread.

\begin{lemma}[Lemma 2.11 of \cite{GuruswamiLR10}]  \label{lem:spread-distortion}
    Let $X\subseteq \R^n$ be a subspace.
    \begin{enumerate}[(1)]
        \item If $X$ is $(t,\eps)$-spread, then $\Delta(X) \leq \sqrt{\frac{n}{t}} \cdot \eps^{-2}$.
        \item Conversely, $X$ is $\parens*{\frac{n}{2\Delta(X)^2}, \frac{1}{4\Delta(X)}}$-spread.
    \end{enumerate}
\end{lemma}



